Exponentials form a basis of discrete holomorphic functions

We show that discrete exponentials form a basis of discrete holomorphic functions. On a convex, the discrete polynomials form a basis as well.

==> dessins/TT <==
\begin{picture}(0,0)%
\includegraphics{dessins/TT.eps}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(6821,2765)(210,-2716)
\put(5008,-1547){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$3$}}}
\put(5331,-406){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$3$}}}
\put(6126,-2319){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$4$}}}
\put(6426,-1367){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$4$}}}
\put(518,-2094){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$0$}}}
\put(1163,-511){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$0$}}}
\put(3714,-2624){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$2$}}}
\put(2668,-1366){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$1$}}}
\put(3934,-389){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$2$}}}
\put(4034,-1607){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$2$}}}
\end{picture}


==> dessins/hexatri <==
\begin{picture}(0,0)%
\includegraphics{dessins/hexatri.eps}%
\end{picture}%
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(8583,7041)(441,-7206)
\end{picture}

